Shattering, Graph Orientations, and Connectivity

We present a connection between two seemingly disparate fields: VC-theory and graph theory. This connection yields natural correspondences between fundamental concepts in VC-theory, such as shattering and VC-dimension, and well-studied concepts of graph theory related to connectivity, combinatorial optimization, forbidden subgraphs, and others. In one direction, we use this connection to derive results in graph theory. Our main tool is a generalization of the Sauer-Shelah Lemma. Using this tool we obtain a series of inequalities and equalities related to properties of orientations of a graph. Some of these results appear to be new, for others we give new and simple proofs. In the other direction, we present new illustrative examples of shattering-extremal systems - a class of set-systems in VC-theory whose understanding is considered by some authors to be incomplete. These examples are derived from properties of orientations related to distances and flows in networks.

==> section5.tex <==
\section{SE systems of orientations} \label{sec5}

An alternative characterization was given independently by Lawrence~\cite{Law}, and by Bollob{\'a}s and Radcliffe~\cite{BR95}. To formalize this characterization, we introduce the following concepts: Let $X$ be a set, given $Y\subseteq X$, a $Y$-\emph{cube} of $\{0,1\}^X$ is an equivalence class of the following equivalence relation on $\{0,1\}^X$: \ \  \framebox{$u\sim v$: ``$u$ agrees with $v$ on $X-Y$''}. A \emph{cube} of $\{0,1\}^X$ is a $Y$-cube for some $Y\subseteq X$. Given $C$, a $Y$-cube of $\{0,1\}^X$, we define $\dim(C) = Y$. Note that the number of $Y$-cubes is $2^{|X-Y|}$, they are mutually disjoint and they cover $\{0,1\}^X$.

Let ${\s=\system{S}{X}}$ be a system and $C \subseteq C(\s)$ be a cube. It is useful to consider the structure $\systemexp{S(\s) \cap C}{C}$ as a system. However, formally it is not a system. To deal with this technicality we give the following definition: The \emph{restriction} of $\s$ to $C$ is the system ${\system{Q}{\dim(C)}}$ where $Q = \setdef{\left.f\right|_{\dim(C)} }{f\in S\cap C}$. A system is a \emph{restriction} of $\s$ if it is a restriction of $\s$ to some cube $C\subseteq C(\s)$.

We define the \emph{antipodal} system of $\s$ as $\ap(\s) = \system{\bar{S}}{X}$, where $\bar{S} = \setdef{f}{1-f \in S}$. A system $\s$ is \emph{symmetric}, if $\s = \ap(\s)$.
 
\begin{theorem}[Lopsidedness~\cite{Law,BR95}]\label{thm:lopsidedness}
A system $\s$ is $SE$, iff it has no non-trivial, symmetric restrictions.  ~\hfill\qed
\end{theorem}
Note that all the systems that we discussed in Section \ref{sec3} are symmetric and thus they are $SE$ if and only if they are trivial.

\laszlo{Should say: many other stuff is known about SE systems, but for the purposes of this paper, this is all we need, for the rest we refer to other papers. Maybe should mention some trivial systems that are SE, e.g. cubes, up/down-closed systems, but say that we look for nontrivial ones.}
\shay{Moreover: we shoud quote Bollobas regarding the hardness of these systems.}


Discussion of SE systems of orientations: including Bollobas charac-
terization and flow orientations

\laszlo{TODO:}\\

* some examples: flow, distance, etc.?

* elaborate on "="\\

* talk about interesting families of SE systems (union, intersection, product operator(?), restriction(?))\\

* talk about SE systems forming partial cube w.r. to Hamming=1 pairs, and what this means for orientations\\

* mention McDiarmid result/Bernardi result for s-W, etc.\\

* inequalities for H-free orientations/H-free graphs\\



